LatteGAN: Visually Guided Language Attention for Multi-Turn Text-Conditioned Image Manipulation

Text-guided image manipulation tasks have recently gained attention in the vision-and-language community. While most of the prior studies focused on single-turn manipulation, our goal in this paper is to address the more challenging multi-turn image manipulation (MTIM) task. Previous models for this task successfully generate images iteratively, given a sequence of instructions and a previously generated image. However, this approach suffers from under-generation and a lack of generated quality of the objects that are described in the instructions, which consequently degrades the overall performance. To overcome these problems, we present a novel architecture called a Visually Guided Language Attention GAN (LatteGAN). Here, we address the limitations of the previous approaches by introducing a Visually Guided Language Attention (Latte) module, which extracts fine-grained text representations for the generator, and a Text-Conditioned U-Net discriminator architecture, which discriminates both the global and local representations of fake or real images. Extensive experiments on two distinct MTIM datasets, CoDraw and i-CLEVR, demonstrate the state-of-the-art performance of the proposed model.

==> tables/results.tex <==
\begin{table*}[tb]
\centering
%\footnotesize
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
           & \multicolumn{4}{c}{CoDraw}            & \multicolumn{1}{l}{} & \multicolumn{4}{c}{i-CLEVR}           \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Methods      & AP$\uparrow$ & AR$\uparrow$ & F1$\uparrow$ & RSIM$\uparrow$  &
& AP$\uparrow$ & AR$\uparrow$ & F1$\uparrow$ & RSIM$\uparrow$  \\ \midrule

% fixed (paper result)
GeNeVA-GAN~{\citep{el2019tell}} & 66.64     & 52.66  & 58.83    & 35.41 &                      & 92.39     & 84.72  & 88.39    & 74.02 \\ \midrule

% fixed (single run, actual results)
% Ours (w/o Latte \& TxtCond)   & 75.33  & 74.05  & 71.98  & 47.13  & & 95.19  & 93.92  & 94.45  & 78.28  \\
Ours (w/o Latte \& TxtCond)
& $76.75{\scriptscriptstyle \pm0.94}$    
& $73.99{\scriptscriptstyle \pm0.11}$ 
& $72.81{\scriptscriptstyle \pm0.51}$
& $47.43{\scriptscriptstyle \pm0.28}$  &
& $95.77{\scriptscriptstyle \pm0.59}$
& $94.60{\scriptscriptstyle \pm0.69}$
& $95.08{\scriptscriptstyle \pm0.65}$
& $79.31{\scriptscriptstyle \pm1.23}$ \\

% temporal (single run, expected results (+4, -1, +2, +.5, +3.5, +4, +4, +5))
% \txq{w/o Latte}        & 79.33  & 73.05  & 73.98  & 47.63  & & 98.69  & 97.92  & 98.45  & 83.28  \\
% Ours (w/o Latte)              & 77.82  & 73.54  & 73.03  & 47.96  & & \bf{98.91}  & \bf{98.58}  & \bf{98.72}  & \bf{83.95}  \\
Ours (w/o Latte)
& $79.04{\scriptscriptstyle \pm1.28}$    
& $73.91{\scriptscriptstyle \pm0.53}$ 
& $74.02{\scriptscriptstyle \pm1.03}$
& $48.16{\scriptscriptstyle \pm0.41}$  &
& $\bm{98.35}{\scriptscriptstyle \pm1.27}$
& $\bm{97.68}{\scriptscriptstyle \pm1.61}$
& $\bm{97.96}{\scriptscriptstyle \pm1.47}$
& $\underline{82.78}{\scriptscriptstyle \pm1.94}$ \\

% fixed (single run, actual results)
% Ours (w/o TxtCond)            & \bf{81.48}  & \bf{78.33}  & \bf{77.51}  & 53.41  & & 96.32  & 95.20  & 95.67  & 80.21  \\
Ours (w/o TxtCond)
& $\underline{80.53}{\scriptscriptstyle \pm0.97}$    
& $\bm{78.42}{\scriptscriptstyle \pm0.38}$ 
& $\underline{77.11}{\scriptscriptstyle \pm0.60}$
& $\underline{53.13}{\scriptscriptstyle \pm0.25}$  &
& $96.67{\scriptscriptstyle \pm0.41}$
& $95.52{\scriptscriptstyle \pm0.43}$
& $95.99{\scriptscriptstyle \pm0.42}$
& $81.04{\scriptscriptstyle \pm0.97}$ \\

% temporal (multiple run, expected results (+4, -1, +2, +.5, +3.5, +4, +4, +5))
% \txq{\bf{LatteGAN (Ours)}}
% & ${85.48}{\scriptscriptstyle \pm0.00}$    
% & ${77.33}{\scriptscriptstyle \pm0.00}$ 
% & ${79.51}{\scriptscriptstyle \pm0.00}$
% & ${53.91}{\scriptscriptstyle \pm0.00}$  &
% & ${99.82}{\scriptscriptstyle \pm0.00}$
% & ${99.20}{\scriptscriptstyle \pm0.00}$
% & ${99.67}{\scriptscriptstyle \pm0.00}$
% & ${85.21}{\scriptscriptstyle \pm0.00}$ \\ \bottomrule
\bf{Ours (LatteGAN)}
& $\bm{81.50}{\scriptscriptstyle \pm0.82}$    
& $\underline{78.37}{\scriptscriptstyle \pm0.38}$ 
& $\bm{77.51}{\scriptscriptstyle \pm0.52}$
& $\bm{54.16}{\scriptscriptstyle \pm0.21}$  &
& $\underline{97.72}{\scriptscriptstyle \pm1.44}$
& $\underline{96.93}{\scriptscriptstyle \pm1.64}$
& $\underline{97.26}{\scriptscriptstyle \pm1.56}$
& $\bm{83.21}{\scriptscriptstyle \pm1.70}$ \\ \bottomrule

\end{tabular}
\end{adjustbox}
\caption{
\textbf{Quantitative comparison and ablation studies.}
The methods have been compared on the CoDraw and i-CLEVR datasets according to several metrics:
the average precision~(AP), average recall (AR), F1-score, and relational similarity (RSIM).
For each metric and dataset, the best scores are in bold,
and the second best ones are underlined.
The mean and standard deviation have been calculated on five different seed runs.
% For i-CLEVR, our model boosted the recall by 12.4 point,
% which resulted in the F1 and RSIM are also improved. 
}\label{tab:results}
\end{table*}
